Discovering the Ethereum2 P2P Network

Achieving the equilibrium between scalability, sustainability, and security while keeping decentralization has prevailed as the target solution for decentralized blockchain applications over the last years. Several approaches have been proposed by multiple blockchain teams to achieve it, Ethereum being among them. Ethereum is on the path of a major protocol improvement called Ethereum 2.0 (Eth2), implementing Sharding and introducing the Proof-of-Stake (PoS). As the change of consensus mechanism is a delicate matter, this improvement will be achieved through different phases, the first of which is the implementation of the Beacon Chain. As Ethereum1, Eth2 relies on a decentralized peer-to-peer (p2p) network for the message distribution. Up to date, we estimate that there are around 5.000 nodes in the Eth2 main net geographically distributed. However, the topology of this one still prevails unknown. In this paper, we present the results obtained from the analysis we performed on the Eth2 p2p network. Describing the topology of the network, as possible hazards that this one implies.

==> future-work.tex <==
\section{Future Work}
\label{sec:futurework}

Rumor is a tool with a huge potential that is still on a development stage. There are still many things to include and improve, this modifications could increase the customization level of the host, increase the Eth2 functionalities that Rumor can support and increase the range of metrics we are gathering, allowing to get a better overview of the healthiness of the Eth2 network.

Between the ideas that has already been discussed, these are the most remarkable ones:
\begin{itemize}
    \item In collaboration with the main developer and maintainer of the Rumor repository @Protolambda, we are working on a new functionality that would allow the custom hosts of Rumor to download and store the messages that we receive from the GossipSub implementation. With this new feature, the custom host would be able to store and serve messages as:
    \begin{itemize}
        \item Block from the Beacon Chain.
        \item States from the Beacon Chain
    \end{itemize}
    The idea behind this functionality would be to evolve Rumor from a p2p custom host to a node that supports the minimum protocols and functionalities from Eth2, allowing the researching/developer community to fake a Eth2 client. This wouldn't mean that you could take Rumor as a valid Beacon-Node option if you wanted to run a eth2 validator. This fake client would offer the chance to keep connected to the peers of the network without experiencing connection drops, increasing the amount of purposes that Rumor can be used for. As an example, the community would have the tool to set up a custom client that could be used to try attacks on the Eth2 network from a malicious beacon node perspective, without needing to modify one of the existing clients and with all the capabilities that a Eth2 client has (sending messages, blocks, states, etc...).
    \item The team is currently working on a modification of the PubSub and GossipSub protocol implementation that would offer the chance to set or not the metadata and message forwarding. With these changes, analyzing the reaction and behavior of the network when it faces a non-honest node would be possible, looking for any possible backdoor that could be used for a network attack.
    \item The team has also in mind to modify the metrics gathering strategy, offering a database of the tracked events as well as all the messages and information gathered by the crawler. Opening the chance to develop Armiarma-Analyzer into a real-time network monitor tool.
\end{itemize}
